The Rationale behind the Concept of Goal

The paper proposes a fresh look at the concept of goal and advances that motivational attitudes like desire, goal and intention are just facets of the broader notion of (acceptable) outcome. We propose to encode the preferences of an agent as sequences of "alternative acceptable outcomes". We then study how the agent's beliefs and norms can be used to filter the mental attitudes out of the sequences of alternative acceptable outcomes. Finally, we formalise such intuitions in a novel Modal Defeasible Logic and we prove that the resulting formalisation is computationally feasible.

==> macro.tex <==

% \usepackage{mathptmx}       % selects Times Roman as basic font
\usepackage{helvet}         % selects Helvetica as sans-serif font
%\usepackage{courier}        % selects Courier as typewriter font
\usepackage{type1cm}        % activate if the above 3 fonts are
                            % not available on your system
%
\usepackage{makeidx}         % allows index generation
\usepackage{graphicx}        % standard LaTeX graphics tool
                             % when including figure files
\usepackage{multicol}        % used for the two-column index
% \usepackage[bottom]{footmisc}% places footnotes at page bottom

% see the list of further useful packages
% in the Reference Guide

%%%%%%%%%%%%%%%
% NINO PACKAGES
%%%%%%%%%%%%%%%

%\usepackage[authoryear]{natbib}
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
%\usepackage{mathptmx}
\usepackage{xspace}
\usepackage{latexsym}
\usepackage{enumerate}
%\usepackage{pdfsync}
\usepackage{tikz}
\usepackage{wrapfig}
\usepackage{subfigure}
%\usepackage{pgf,pgfarrows,pgfnodes,pgfautomata,pgfheaps,pgfshade}
\usepackage{color}
%\usepackage{colortbl}

\usepackage{qtree}


%%%%%%
\usepackage{latexsym,verbatim}
\usepackage{amsmath}
% \usepackage{mathptmx}
\usepackage{amssymb}
\usepackage{xspace}
\usepackage{alltt}
%%%%%%

%\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{algorithmic}

\usepackage{xspace}
\usepackage{latexsym}
%\usepackage{pdfsync}
\usepackage{tikz}

%%%%%%%%%%%%%%%%%%%%%
% NINO COMMANDS
%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ann}{\ensuremath{\mathrm{annul}}\xspace}
\newcommand{\sub}{\ensuremath{\mathrm{subst}}\xspace}
\newcommand{\tsub}{\ensuremath{\mathrm{TSubstitution}}\xspace}
\newcommand{\der}{\ensuremath{\mathrm{derog}}\xspace}
\newcommand{\abrog}{\ensuremath{\mathrm{abrog}}\xspace}
\newcommand{\non}{\mathnormal{\sim}}

\newcommand{\FACTS}{\ensuremath{\mathrm{F}}\xspace}
\newcommand{\OBL}{\ensuremath{\mathrm{O}}\xspace}
\newcommand{\BEL}{\ensuremath{\mathrm{B}}\xspace}
\newcommand{\GOAL}{\ensuremath{\mathrm{G}}\xspace}
\newcommand{\DES}{\ensuremath{\mathrm{D}}\xspace}
\newcommand{\INT}{\ensuremath{\mathrm{I}}\xspace}


\newcommand{\Convert}{\ensuremath{\mathrm{Convert}}\xspace}
\newcommand{\Conflict}{\ensuremath{\mathrm{Conflict}}\xspace}

\newcommand{\Aconf}[2]{\mathrm{Conflict}(#1,#2)}
\newcommand{\Aconv}[2]{\mathrm{Convert}(#1,#2)}
\newcommand{\ds}{\displaystyle}
\newcommand{\oseq}[2][n]{#2_{1}\odot\cdots\odot #2_{#1}}
\newcommand{\opseq}[4][\otimes]{#2_{#3}#1\cdots#1#2_{#4}}

\newcommand{\defeater}{\leadsto}

\newcommand{\seqm}[2][m]{\ensuremath{#2_1,\dots,#2_{#1}}}

\newcommand{\inP}{\in P[1..n]}
\newcommand{\Rnon}{R^{\mathrm{nm}}} %non modifiable rules
\newcommand{\metaR}{R^{\mathrm{meta}}} %meta-rules
\newcommand{\Rmod}{R^{\mathrm{mod}}} % modifiable rules
\newcommand{\set}[2][\relax]{\ensuremath{#1\{#2#1\}}}
\newcommand{\Set}[2][\relax]{%
  \ensuremath{
    \ifx#1\left
      #1\{#2\right\}
    \else\ifx#1\right
      \left\{#2#1\}
      \else #1\{#2#1\}\fi\fi}%
}
\RequirePackage{ifthen}
\renewcommand{\Set}[2][\relax]{%
  \ifthenelse{\equal{#1}{auto}}{\left\{#2\right\}}{#1\{#2#1\}}%
}
\newcommand{\seq}[2][n]{\ensuremath{#2_1,\dots,#2_{#1}}}
\newcommand{\cT}{\ensuremath{\mathcal{T}}}
\newcommand{\TLit}{\ensuremath{\mathrm{TLit}}}
\newcommand{\Rules}{\ensuremath{\mathrm{Rules}}}

\newcommand{\To}{\Rightarrow}

\usetikzlibrary{shapes}
\newcommand{\printdb}[1]{LS(#1)}

\let\arrow\hookrightarrow

\newcommand{\red}[1]{{\color{red} #1}}


